Study of the spin and parity of the Higgs boson in diboson decays with the ATLAS detector

Studies of the spin, parity and tensor couplings of the Higgs boson in the $H\rightarrow ZZ^*\rightarrow 4\ell$, $H\rightarrow WW^* \rightarrow e\nu\mu\nu$ and $H\rightarrow \gamma \gamma$ decay processes at the LHC are presented. The investigations are based on $25$ fb$^{-1}$ of $pp$ collision data collected by the ATLAS experiment at $\sqrt{ s} = 7$ TeV and $\sqrt{ s }= 8$ TeV. The Standard Model (SM) Higgs boson hypothesis, corresponding to the quantum numbers $J ^P=0^+$, is tested against several alternative spin scenarios, including non-SM spin-0 and spin-2 models with universal and non-universal couplings to fermions and vector bosons. All tested alternative models are excluded in favour of the SM Higgs boson hypothesis at more than 99.9% confidence level. Using the $H\rightarrow ZZ^*\rightarrow 4\ell$ and $H\rightarrow WW^* \rightarrow e\nu\mu\nu$ decays, the tensor structure of the $HVV$ interaction in the spin-0 hypothesis is also investigated. The observed distributions of variables sensitive to the non-SM tensor couplings are compatible with the SM predictions and constraints on the non-SM couplings are derived.

==> summary.tex <==
The distributions of $\Delta \ln L $ for the  of $\KtildeH$ and $\KtildeA$ 
measured in the \hZZ\ analysis are shown in Figure~\ref{fig:res_cond}.
\begin{figure*}[htbp]
 \centering
\begin{minipage}[h]{0.45\linewidth}
\center{\includegraphics[width=1.0\linewidth]{figures/hzz/mixing/loglambdaScan_Run1_fit_g2_fullSyst}}  
\end{minipage}
\hfill
\begin{minipage}[h]{0.45\linewidth}
\center{\includegraphics[width=1.0\linewidth]{figures/hzz/mixing/loglambdaScan_Run1_fit_g4_fullSyst}}  
\end{minipage}
   \caption{ \label{fig:res_cond}  Expected and observed  
distributions of   $\Delta \ln L $ for the  fits of $\KtildeH$ (left) and $\KtildeA$ (right), for $H\to ZZ^* \to 4\ell$ analysis.
The expected curves are  calculated assuming the Standard Model $J^P=0 ^+$ signal and  produced with the Standard Model 
signal strength $\mu =1$ and with the signal strength fitted to data: $\hat{\mu}$.  The horizontal dotted black lines represent the 
levels of $\Delta \ln L $ above which the values of coupling ratios under study are excluded above $68$ and $95\%$~CL.} 
\end{figure*}
he expected curves are  calculated assuming the Standard Model $J^P=0 ^+$ signal and  produced with the Standard Model 
signal strength $\mu =1$ and with the signal strength fitted to data: $\hat{\mu}$. The effects of systematic  
uncertainties listed above are taken into account during the fit. The fitted values of 
$g_2/g_1$ and $g_4/g_1$ together with the intervals where these couplings are excluded 
above  $95\%$~CL, are reported in Table~\ref{tab:res_cond}.
\begin{table}
\centering
 \begin{tabular}{lccc}
 \hline\hline
Coupling ratio & Best fit value & \multicolumn{2}{c}{$95\%$CL Exclusion Regions} \\
 &&Expected&Observed\\
 \hline
 $\KtildeH$ & $0.0$ & & $[-1.88;-0.88]$\\
 $\KtildeA$ & $0.0$ & & $(-\inf;-5.22]\cup[5.17,+\inf)$\\
   \hline\hline
 \end{tabular}
\caption{\label{tab:res_cond} Fitted values of $\KtildeH$ and $\KtildeA$ and  $95\%$~CL excluded regions obtained in $H\to ZZ^* \to 4\ell$ analysis.}
\end{table}
It is noted that the fitted values agree with the Standard Model predictions within the calculated
uncertainties. 

\begin{figure}[htbp]
  \centering
  \subfloat{\includegraphics[width=0.49\textwidth]{figures/dummyPlot}}
  \subfloat{\includegraphics[width=0.49\textwidth]{figures/dummyPlot}}\\
  
  \caption{The $95\%$~CL exclusion regions for BSM CP-odd (left) and CP-even (right) 
  couplings obtained in $H\to ZZ^*\to 4 \ell$ and $H\to WW \to \ell \nu\ell\nu$ analyses. \label{fig:tensor_correlation}}
\end{figure}

\begin{figure}[htbp]
  \centering
  \subfloat{\includegraphics[width=0.49\textwidth]{figures/dummyPlot}}
  \subfloat{\includegraphics[width=0.49\textwidth]{figures/dummyPlot}}\\
  
  \caption{The BSM CP-odd (left) and CP-even (right) combined scan results. The -2$\Delta$Log(L) scan
    is shown as a function of each of the two mixing parameters. The 68\% and 95\% CL exclusion regions
    are indicated as lyinga bove the corresponding horizontal lines\label{fig:tensor_logl}.}
    
\end{figure}

\begin{table}[ht]
\centering
\begin{tabular} {lccc}
\hline
\hline
 Coupling ratio & Best fit value & \multicolumn{2}{c}{$95\%$CL Exclusion Regions} \\
 &&Expected&Observed\\
\hline
 $\KtildeA$          &   &  &   \\                          
 $\KtildeH$          &   &  &   \\                          
                                                                                         
\hline
\hline
\end{tabular}
\caption{Expected and observed mixing parameters excluded regions, for the combination of the 
$H\to ZZ^*\to 4 \ell$  and $H\to WW \to \ell \nu\ell\nu$ channels. The excluded regions are computed at 95\% CL.\label{tab:mixing_exclusion} }
\end{table}                                    

